Adaptable Teastore with Energy Consumption Awareness: A Case Study

[Context and Motivation] Global energy consumption has been steadily increasing in recent years, with data centers emerging as major contributors. This growth is largely driven by the widespread migration of applications to the Cloud, alongside a rising number of users consuming digital content. Dynamic adaptation (or self-adaptive) approaches appear as a way to reduce, at runtime and under certain constraints, the energy consumption of software applications. [Question/Problem] Despite efforts to make energy-efficiency a primary goal in the dynamic adaptation of software applications, there is still a gap in understanding how to equip these self-adaptive software systems (SAS), which are dynamically adapted at runtime, with effective energy consumption monitoring tools that enable energy-awareness. Furthermore, the extent to which such an energy consumption monitoring tool impacts the overall energy consumption of the SAS ecosystem has not yet been thoroughly explored. [Methodology] To address this gap, we introduce the EnCoMSAS (Energy Consumption Monitoring for Self-Adaptive Systems) tool that allows to gather the energy consumed by distributed software applications deployed, for instance, in the Cloud. EnCoMSAS enables the evaluation of energy consumption of SAS variants at runtime. It allows to integrate energy-efficiency as a main goal in the analysis and execution of new adaptation plans for the SAS. In order to evaluate the effectiveness of EnCoMSAS and investigate its impact on the overall energy consumption of the SAS ecosystem, we conduct an empirical study by using the Adaptable TeaStore case study. Adaptable TeaStore is a self-adaptive extension of the TeaStore application, a microservice benchmarking application. For this study, we focus on the recommender service of Adaptable TeaStore. Regarding the experiments, we first equip Adaptable TeaStore with EnCoMSAS. Next, we execute Adaptable TeaStore by varying workload conditions that simulate users interactions. Finally, we use EnCoMSAS for gathering and assessing the energy consumption of the recommender algorithms of Adaptable TeaStore. To run these experiments, we use nodes of the Grid5000 testbed. [Results] The results show that EnCoMSAS is effective in collecting energy consumption of software applications for enabling dynamic adaptation at runtime. The observed correlation between CPU usage and energy consumption collected by EnCoMSAS provides evidence supporting the validity of the collected energy measurements. Moreover, we point out, through EnCoMSAS, that energy consumption is influenced not only by the algorithmic complexity but also by the characteristics of the deployment environment. Finally, the results show that the impact of EnCoMSAS on the overall energy consumption of the SAS ecosystem is comparatively modest with respect to the entire set of the TeaStore applications microservices.

==> eptcsdata.tex <==
\providecommand{\firstpage}{100}
\providecommand{\publicationstatus}{G. De Palma and S. Giallorenzo (Eds.):\\
First Workshop on Adaptable Cloud Architectures\\
EPTCS 438, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.438.6}{10.4204/EPTCS.438.6}}
\pdfoutput=1
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{6}}{\finishreference{#1}{438}{\opa}{79}{99}{5}}{%
 this volume of #1\opa}}


==> sections/abstract.tex <==
Global energy consumption has been steadily increasing in the recent years, with data centers emerging as major contributors. This growth is largely driven by the widespread migration of applications to the Cloud, alongside a rising number of users consuming digital content. 
One way for reducing the energy consumption of data centres involves improving the energy efficiency of the deployed software applications. This implies design time and runtime approaches with self-adaptive applications.
Although various strategies have been proposed, there is limited research comparing the architectural tactics employed in self-adaptive applications. In particular, there is a lack of evaluation regarding the energy consumption impact of architectural variants proposed in Cloud applications.

To address this gap, we propose a framework to integrate variants in the implementation of applications and allow to choose one particular variant according to its associated energy consumption at runtime. We add a monitor component to a Cloud application to track the energy usage of application containers and select adaptations according to the energy consumption of a microservice.

We have performed an empirical study on the Adaptable TeaStore application in a scenario of workload traffic on a node within the Grid5000 testbed. 
We assess the energy consumption of variants of the recommendation algorithm proposed by the TeaStore application, and we propose a functional level adaptation by analysing the behaviour of the application. First results show some potential improvements in the energy efficiency of cloud applications at runtime. 


%%\textbf{Motivation}: %As companies increasingly migrate services to the Cloud, the energy consumption of data centers has grown significantly. Cloud providers are responsible for delivering the necessary infrastructure resources to meet customer demands. The adoption of self-adaptive systems can optimize energy usage from both a hardware provisioning and application architecture perspective, reducing the need for human intervention. 
%Energy efficiency is an important concern when analysing applications running in data centres. %As the global demand for Cloud services continues to grow, so does the energy consumption of Cloud operations, placing increasing strain on environmental resources. 
%While prior work has proposed solutions such as host-level energy monitoring and hardware resource provisioning, we argue that architectural-level analysis can offer valuable insights and contribute to the development of more energy-efficient applications.

%%\noindent\textbf{Problem statement:}
%Although various strategies for developing energy-efficient systems have been proposed, there is limited research comparing the architectural tactics employed by these self-adaptive systems. In particular, there is a lack of evaluation regarding the energy consumption impact of the architectural variants presented in Cloud application.

%%\noindent\textbf{Approach}:
%To address this gap, we analyse the energy consumption of Cloud applications defining an adaptation in the architecture and validating it at runtime. % according to the energy consumption values. 
%We add a monitor component to a Cloud application to track the energy usage of application containers and select a service to provide adaptations according to the energy consumption of a microservice.

%%\noindent\textbf{Method}:
%We perform an empirical study involving the execution of the TeaStore application in a scenario of workload traffic on a node within the Grid5000 testbed tool. %We assess the impact of the recommender algorithms proposed by the application in the energy consumption of all microservices. 
%We assess the impact of the energy consumption of different recommender algorithms proposed by the application, and apply them over a functional level adaptation to analyse the behaviour of the energy consumption of the service. 

%% \textbf{Results}: By analyzing each recommendation algorithm individually, we were able to compare their energy consumption and identify the most efficient option for use within the application. However, our results indicate that selecting the algorithm with the lowest individual energy consumption does not necessarily lead to an overall reduction in the energy consumption of a microservice. But, we consider that the adaptations are carried out by the microservice itself, which requires further studies about this impact.

%\textbf{Conclusion}: 
%Our findings show that selecting energy-efficient algorithms does not necessarily lead to the decrease of overall energy consumption for the application.
%Understanding an application's energy consumption is essential for developing energy-efficient solutions and for improving predictability in areas such as electricity costs. This insight enables more informed decision-making when selecting components and configurations to incorporate into the application.

==> sections/abstract_V2.tex <==
\textbf{[Context and Motivation]}
Global energy consumption has been steadily increasing in recent years, with data centers emerging as major contributors. This growth is largely driven by the widespread migration of applications to the Cloud, alongside a rising number of users consuming digital content. 
One way to reduce the energy consumption of data centers involves improving the energy efficiency of the software applications that are deployed. This implies the incorporation of energy profiling tools and runtime experiments with variants in a self-adaptive application.


\textbf{[Question/Problem]}
Although various strategies have been proposed, there is limited research comparing architectural tactics employed in self-adaptive applications with energy profiling instrumentation. In particular, there is a lack of studies concerning the impact of these energy profiling tools and the impact of different variants in cloud applications on energy consumption.

\textbf{[Methodology]}
To address this gap, we present a case study in a self-adaptive application that integrates an energy consumption profiling framework. This framework enables energy awareness in a cloud application, enabling to find the most energy efficient algorithm at runtime. Specifically, we assess the energy consumption of the recommender algorithms within the Adaptable TeaStore application, under varying workload conditions on a node in the Grid5000 testbed. We compare the energy and complexity of different recommender algorithms proposed by TeaStore and propose a dynamic adaptation strategy focused on energy efficiency. Finally, we evaluate the impact of this framework on overall energy consumption.

\textbf{[Results]}
The results indicate that energy efficiency is influenced not only by the choice of algorithm but also by the characteristics of the deployment environment. Additionally, a strong correlation is observed between CPU usage and energy consumption of the algorithms and the variants.

==> sections/abstract_draft.tex <==
Global energy consumption has been steadily increasing in recent years, with data centers emerging as major contributors. This growth is largely driven by the widespread migration of applications to the Cloud, alongside a rising number of users consuming digital content. 
One way to reduce the energy consumption of data centers involves improving the energy efficiency of the software applications that are deployed. This implies the incorporation of energy profiling tools and runtime experiments with variants in a self-adaptive application.
Although various strategies have been proposed, there is limited research comparing architectural tactics employed in self-adaptive applications with energy profiling instrumentation. In particular, there is a lack of studies concerning the impact of these energy profiling tools and the impact of different variants proposed in cloud applications.
To address this gap, we investigate a case study with a self-adaptive application, incorporating an energy consumption profiling monitor framework, analyzing its impact, and integrating variants, allowing us to choose one particular variant according to its associated energy consumption at runtime.
We analyze the energy consumption of the recommender microservice of Adaptable TeaStore in a scenario of workload traffic on a node within the Grid5000 testbed. We assess the energy consumption of different recommender algorithms proposed by the TeaStore application, propose dynamic adaptation concerning energy efficient adaptation, and evaluate the impact of the solution on overall energy consumption. Results show that the energy efficiency depends not only on the most energy efficient algorithm, but also on the deployment environment.
